Adapting to Distribution Shift by Visual Domain Prompt Generation

In this paper, we aim to adapt a model at test-time using a few unlabeled data to address distribution shifts. To tackle the challenges of extracting domain knowledge from a limited amount of data, it is crucial to utilize correlated information from pre-trained backbones and source domains. Previous studies fail to utilize recent foundation models with strong out-of-distribution generalization. Additionally, domain-centric designs are not flavored in their works. Furthermore, they employ the process of modelling source domains and the process of learning to adapt independently into disjoint training stages. In this work, we propose an approach on top of the pre-computed features of the foundation model. Specifically, we build a knowledge bank to learn the transferable knowledge from source domains. Conditioned on few-shot target data, we introduce a domain prompt generator to condense the knowledge bank into a domain-specific prompt. The domain prompt then directs the visual features towards a particular domain via a guidance module. Moreover, we propose a domain-aware contrastive loss and employ meta-learning to facilitate domain knowledge extraction. Extensive experiments are conducted to validate the domain knowledge extraction. The proposed method outperforms previous work on 5 large-scale benchmarks including WILDS and DomainNet.

==> Old/Intro.tex <==
\section{Introduction}
% In this section, we describe Distribution Shifts, Domain Generalization, and our few-shot Test-time domain adaptation (FS-TT-DA)
The superior performance of deep models relies on the assumption that both training and testing data examples are drawn from the identical data distribution. However, in the real world, the training data may not contain the prior knowledge of an infinite of testing scenarios, and thus models confront the issue of performance degradation when deployed at test-time, known as distribution shifts \cite{koh2021wilds}. To improve model robustness against distribution shift, Domain Generalization\cite{pmlr-v28-muandet13, ghifary2015domain, balaji2018metareg} aims to leverage one or multiple source domains to learn domain-invariant knowledge that could generalize well to any unseen target domain. Nevertheless, a lack of domain-specific knowledge of the target domain hinders the model from achieving the optimal \cite{sun2020test}.
Alternatively, a limited amount of unlabeled data examples from the target domain is readily accessible at test-time. These few-shot examples can be collected to guide the pre-trained model to adapt to the target domain before making inferences on the remaining examples \cite{zhong2022meta}, similar to the process of camera calibration.

A well-designed mechanism for test-time domain adaptation with few-shot unlabeled data examples should carefully address three fundamental challenges. 1) how to effectively learn the domain knowledge that can be transferable from multi-source domains to any unseen target domain? 2) how to acquire valid domain-specific knowledge for the target domain by combining the knowledge extracted from the few-shot target data with the knowledge transferred from multi-source domains? 3) how to efficiently guide the pretrained model using the target domain knowledge? \cite{zhong2022meta} encodes the multi-source domain knowledge into a mixture of expert teacher networks. Given a target domain, a few unlabeled data are collected to query the transferable knowledge that supervises the adaptation of a student network via fine-tuning. However, storing domain knowledge in the parameter space of a mixture of networks introduces heavy computation and storage overheads that scale linearly with the number of source domains \cite{shazeer2017, puigcerver2023sparse}. Moreover, fine-tuning the entire network during test-time adaptation requires abundant memory space and power consumption, and is thus unfriendly to resource-constrained devices \cite{NEURIPS2020_81f7acab, NEURIPS2022_90c56c77}.

Alternatively, following the recent trend in Prompt Tuning \cite{lester-etal-2021-power, li-liang-2021-prefix, liu2022p} in NLP, Visual Prompt Tuning \cite{bahng2022exploring, jia2022visual, Wang_2022_CVPR, wang2022dualprompt, han2023e2vpt} provides a parameter-efficient fine-tuning framework to handle distribution shifts. In visual prompting, an ImageNet-pre-trained backbone can be guided to adapt to a downstream image classification dataset by optimizing the learnable prompt tokens prepended to the image input instead of optimizing the entire network. Inspired by this, source domain knowledge is embedded into learnable prompt tokens. During adaptation, a target domain prompt is generated based on the unlabeled data while the backbone parameters are frozen \cite{zheng2022prompt, gao2022visual, gan2023decorate}. This also enables the modification of domain knowledge exclusively within the input space instead of the parameter space. In \cite{zheng2022prompt}, the knowledge of multi-source domains is individually encoded into distinct domain prompts corresponding to each source dataset. A target prompt is then produced by analyzing the domain distance between learned source prompts and the target input feature.
In \cite{gan2023decorate}, a source domain prompt is heuristically partitioned into domain-specific and domain-shareable components, with initialization via supervised learning on multi-source domain datasets. To facilitate knowledge transfer during adaptation, a manually crafted regularization term is employed to preseve the domain-shareable while allowing the domain-specific updates.


However, these recent approaches have multiple major drawbacks. First, as the modeling of source domain knowledge relies solely on the cross-entropy loss, the domain prompt may inadvertently learn patterns of semantic categories because it is a shortcut to fulfill the classification requirement \cite{li2023rethinking}. Second, separating the modeling of source knowledge and the extraction of target knowledge into independent training phases may compromise optimal knowledge transfer to the target domain. Last, all previous methods opt to finetune the backbone network on multi-source domain datasets to boost performance. This strategy incurs prohibitive training costs and becomes increasingly impractical as the size of backbone networks continues to grow \cite{pmlr-v202-dehghani23a}.

In this work, we propose a novel approach that aims to use the visual prompt and the large foundation model \cite{bommasani2021opportunities} (e.g., CLIP \cite{radford2021learning}) to address distribution shifts. We assume that the highly generalized features intrinsic to the foundation model can be manipulated to adapt to any domain by incorporating corresponding domain-specific knowledge. The key idea is to generate a domain-specific visual prompt from few-shot unlabeled data to provide guidance to the foundation model. Specifically, we propose a domain prompt generator in which a learnable knowledge bank is designed to encode transferable knowledge from multiple source domains. Given a target domain, the prompt generator takes as input a mini-batch of unlabeled data to condense the knowledge bank into a domain-specific prompt. This domain prompt is then incorporated into the foundation model via a guidance module. To purify the domain-specific knowledge without semantic interference, we introduce a domain-aware contrastive loss to supervise the prompt generator. This also allows us to exploit large-scale unlabeled data only with domain IDs \cite{sagawa2022extending} to further improve generalization. Moreover, to learn the transferable knowledge and the mechanism of adaptation simultaneously, we employ episodic learning to train the prompt generator and the guidance module at the meta-level \cite{hospedales2021meta}. Furthermore, to minimize the training cost and maintain the out-of-distribution generalization \cite{Wortsman_2022_CVPR}, we do not fine-tune the foundation model in both training and adaptation. 
 
Our proposed method also provides additional practical advantages. As the domain prompt is the output embedding from the prompt generator, it is unnecessary to backpropagate the gradients through the foundational model. This feature allows our prompt generator can be readily integrated with commercially available foundational models via APIs in a black-box setting \cite{ouali2023black}, significantly reducing memory overheads and privacy leaks \cite{xu2020information}. Furthermore, generating a target domain prompt at test time is gradient-free, making it well-suited for on-device deployment scenarios.

We summarize our main contributions as follows: 1) We propose a novel framework that employs visual prompting to tackle distribution shifts. Our approach formulate the adaptation process as generating a visual prompt that encodes domain-specific knowledge to guide the foundational model. 2) Our method offers multiple practical benefits, including computational efficiency, low memory consumption during both training and deployment, and privacy guarantee 3) We conduct extensive experiments to show the superiority of the proposed method among the state-of-the-art and verify the effectiveness of each component. 
 




==> Old/Intro_v0.tex <==
\section{Introduction}
% In this section, we describe the problem setting and the motivations for our domain adaptive method. 
The superior performance of deep models relies on the strong assumption that both training and testing data examples are drawn from identical data distribution. However, in real-world settings, the training data may not contain the prior knowledge of an infinite of testing scenarios, and thus models may encounter the issue of performance degradation when deployed at test-time, known as distribution shift. To improve model robustness against distribution shift, Domain Generalization (DG) aims to leverage one or multiple source domains to learn domain-invariant knowledge that could generalize well to any unseen target domain. Nevertheless, a lack of domain-specific knowledge of the target domain hinders the model from achieving the optimal. To leverage the knowledge of the target domain, Unsupervised Domain Adaptation (UDA) necessitates access to both labeled source data and unlabeled target data at train-time. However, collecting data from a target domain in advance is impractical and even prohibitive in privacy-sensitive applications. Instead, Test-time adaptation (TTA) allows the model to access unlabeled target data only at test-time, which enables the pre-trained model to adapt to the target domain before making predictions.

A well-designed mechanism for TTA-DA should carefully address two fundamental challenges. First, how can we effectively encode domain-related knowledge so that the semantic knowledge can remain untouchable during adaptation? Encoding knowledge in the model's parameter space, most conventional approaches select a subset of parameters to store domain knowledge. However, it is extremely hard to determine which subset ansize leading to the balance between the limited adaptation capacity and overfitting with few-shot target data. Second, how can we efficiently adapt the model with the domain knowledge from the unlabelled target data? Previous works craft unsupervised objectives, such as self-supervised auxiliary tasks or pseudo labels, to finetune the domain-related subset parameters, but heuristic unsupervised objectives may provide noisy supervision. In addition, finetuning a model after deployment at test-time requires extra abundant computation power and memory space and is thus unfriendly to resource-constrained devices. 

Alternatively, inspired by the success of prompting in NLP, Visual prompting can provide a novel framework for Test-Time Adaptation to address distribution shifts. In visual prompting, a large foundational model (FM)—pretrained on web-scale datasets (e.g.CLIP) and endowed with out-of-distribution generalization—can be steered to perform a downstream task by prepending prompt tokens to the image input instead of optimizing the entire network. Inspired by this, we encode domain-specific knowledge into a prompt and leave the semantic knowledge in the foundation model unspoiled. It assumes the highly generalized feature inherent in the foundation model can be manipulated to adapt to any domain by injecting corresponding domain-specific knowledge. This enables the modification of domain-specific knowledge exclusively within the input space, eliminating the necessity for optimization in the parameter space during adaptation to the target domain. The remaining challenge lies in how to effectively acquire a valid target domain prompt at test-time by combining the domain-specific knowledge extracted from limited unlabeled target data with the domain-sharable knowledge transferred from multi-source datasets. [ ]  first encodes the knowledge of multi-source domains into distinct domain prompts by learning from each source dataset independently, and then learns to aggregate these multiple source prompts into a target prompt by comparing the similarity with the target input feature. [ ] first heuristically partitions the domain prompt into domain-specific and domain-sharable components initialized by supervised learning on multi-source datasets, and then employs a manually designed regularization to preserve the domain-sharable component, thereby facilitating knowledge transfer in the adaptation.

However, these early attempts in visual prompting have multiple major drawbacks. First, both approaches finetune the FM on multi-source datasets, thereby violating the fundamental principle of prompting. This significantly hampers the FM’s intrinsic robustness in handling domain shifts. In addition, finetuning introduces prohibitive training costs and becomes extremely impractical as the size of FMs continues to grow. Second, both solely fullfill the objective of classification when learning the multi-source domain knowledge, potentially capturing shortcut patterns rather than the intrinsic data distribution in the source domain prompts. Last, the modeling process of multi-source domains and the scheme of test-time adaptation are separated into two distinct learning phases. This may not guarantee that the learned knowledge can be optimally transferable to a target domain.


We introduce xxx, a generalized prompting strategy that aims to learn how to learn valid transferable knowledge that can provide guidance to extract target domain knowledge from few-shot unlabeled data without knowing the foundation model's architecture. Concretely, we propose a Prompt Generator designed to integrate a knowledge bank that holds transferrable knowledge across various domains. Given a target domain,  a few unlabeled data are collected to guide the knowledge bank to concentrate on domain-specific knowledge that is used to generate a target domain prompt. A decoder module is proposed to incorporate the domain-specific prompt into the generalized foundational model, facilitating the model's adaptation to the target domain. To learn the sharable domain knowledge and the scheme of knowledge transfer, we employ episodic learning to train the Prompt Generator and the decoder at the meta-level. In addition, the Prompt Generator can fully leverage large-scale unlabeled data with domain IDs to further improve generalization. 

The proposed method also provides additional practical advantages over previous prompting approaches. The domain prompt is the direct output embedding from the Prompt Generator, as opposed to tunable vectors that could be optimized, which eliminates the need for backpropagating the gradients through foundational models. This feature allows the Domain Prompt Generator can be readily integrated with commercially available foundational models via APIs, significantly reducing both computational and memory overhead. Furthermore, generating the target domain prompt at test time is gradient-free and requires only a single forward pass through the Prompt Generator network, making it well-suited for on-device deployment scenarios.

We summarize our main contributions as follows:

We introduce a test-time visual prompt generation approach that is tailored to address distribution shifts. Our framework employs the concept of visual prompting to separate domain-specific knowledge from semantic knowledge. We formulate the adaptation process as generating and incorporating a domain-specific prompt into the foundational model.

We propose a prompt generator to learn the shareable domain knowledge across domains and the mechanism of knowledge transfer via meta-learning without access to the foundation model's parameters. 

We conduct extensive experiments on image classification and regression to show the superiority of the proposed method among the state-of-the-art and validate the effectiveness of each component.



==> Old/Intro_v1.tex <==
\section{Introduction}
% In this section, we describe the problem setting and the motivations for our domain adaptive method. 
The superior performance of deep models relies on the strong assumption that both training and testing data examples are drawn from identical data distribution. However, in real-world settings, the training data may not contain the prior knowledge of an infinite of testing scenarios, and thus models may encounter the issue of performance degradation when deployed at test-time, known as distribution shift. To improve model robustness against distribution shift, Domain Generalization (DG) aims to leverage one or multiple source domains to learn domain-invariant knowledge that could generalize well to any unseen target domain. Nevertheless, a lack of domain-specific knowledge of the target domain hinders the model from achieving the optimal. Instead, Test-time adaptation (TTA) allows the model to access unlabeled target data only at test-time, which enables the pre-trained model to adapt to the target domain before making predictions.

A well-designed mechanism for TTA-DA should carefully address two fundamental challenges. First, how to effectively encode domain-specific knowledge so that the semantic knowledge can remain untouchable during adaptation? Encoding knowledge in the model's parameter space, most conventional approaches select a subset of parameters to store domain knowledge. However, it is extremely hard to specify the subset and its size to achieve a balance between the limited adaptation capacity and overfitting with few-shot target data. Second, how to efficiently adapt the model with the domain knowledge given the limited unlabelled target data? Previous works craft unsupervised objectives, such as self-supervised auxiliary tasks or pseudo labels, to finetune the domain-related subset parameters, but heuristic unsupervised objectives may provide noisy supervision. In addition, finetuning a model after deployment at test-time requires extra abundant computation power and memory space and is thus unfriendly to resource-constrained devices. 

Alternatively, inspired by the success of prompting in NLP, Visual prompting can provide a novel framework for Test-Time Adaptation to address distribution shifts. In visual prompting, a large foundational model (FM)—pretrained on web-scale datasets (e.g.CLIP) and endowed with out-of-distribution generalization—can be steered to perform a downstream task by prepending prompt tokens to the image input instead of optimizing the entire network. Inspired by this, we encode domain-specific knowledge into a prompt and leave the semantic knowledge in the foundation model unspoiled. It assumes the highly generalized feature inherent in the foundation model can be manipulated to adapt to any domain by injecting corresponding domain-specific knowledge. This enables the modification of domain-specific knowledge exclusively within the input space, eliminating the necessity for optimization in the parameter space during adaptation. The remaining challenge lies in how to effectively acquire a valid target domain prompt at test-time by combining the specific knowledge extracted from limited unlabeled target data with the shareable knowledge transferred from multi-source datasets. [ ]  first encodes the knowledge of multi-source domains into distinct domain prompts by learning from each source dataset independently, and then learns to aggregate these multiple source prompts into a target prompt by comparing the similarity with the target input feature. [ ] first heuristically partitions the domain prompt into domain-specific and domain-sharable components initialized by supervised learning on multi-source datasets, and then employs a manually designed regularization to preserve the domain-sharable component, thereby facilitating knowledge transfer in the adaptation.

However, these early attempts in visual prompting have multiple major drawbacks. First, both approaches finetune the FM on multi-source datasets, thereby violating the fundamental principle of prompting. This significantly hampers the FM’s intrinsic robustness in handling domain shifts. In addition, finetuning introduces prohibitive training costs and becomes extremely impractical as the size of FMs continues to grow. Second, both solely fullfill the objective of classification when learning the multi-source domain knowledge, potentially capturing shortcut patterns rather than the intrinsic data distribution in the source domain prompts. Last, the modeling process of multi-source domains and the scheme of test-time adaptation are separated into two distinct learning phases. This may not guarantee that the learned knowledge can be optimally transferable to a target domain.


In this work, we introduce XXX, a novel visual prompting approach that aims to extract domain-specific knowledge from limited unlabeled data to guide the foundation model to adapt to an unseen domain. Concretely, we propose a domain prompt generator in which a learnable knowledge bank is designed to encode transferable knowledge from multiple source domains. Given a target domain, the prompt generator takes as input a mini-batch of unlabeled data to condense the knowledge bank into a domain-specific prompt. To strengthen the domain knowledge condensation without semantic interference , we introduce a domain-aware contrastive loss to supervise the prompt generator. This also allows us to exploit large-scale unlabeled data only with domain IDs to further improve generalization. Moreover, the generated domain prompt is incorporated into the foundation model via a decoding module to guide the adaptation. To learn the knowledge bank and the process of knowledge transfer, we employ episodic learning to train the prompt generator and the decoder module at the meta-level. 

Our proposed method also provides additional practical advantages. As the domain prompt is the output embedding from the Prompt Generator, it is unnecessary to backpropagate the gradients through foundational model to optimize the prompt vectors in Prompt Tuning. This feature allows our Prompt Generator can be readily integrated with commercially available foundational models via APIs in black-box setting, significantly reducing memory overheads and privacy leak. Furthermore, generating the target domain prompt at test time is gradient-free, making it well-suited for on-device deployment scenarios.

We summarize our main contributions as follows: 1) We propose a novel test-time adaptation framework that is tailored to address distribution shifts. Our framework employs the concept of visual prompting and formulate the adaptation process as extracting domain-specific knowledge from unlabeled data into a prompt to guide the foundation model. 2) We design a visual prompt generation approach that aims to learn the process of domain knowledge extraction via meta-learning. Our method is also resource-efficient in training and deployment, as the large models can be treated as a black box without the need to access its internal information. 3) We conduct extensive experiments to show the superiority of the proposed method among the state-of-the-art and verify the effectiveness of each component. 




==> Old/Intro_v2.tex <==
\section{Introduction}
% In this section, we describe Distribution Shifts, Domain Generalization, and our few-shot Test-time domain adaptation (FS-TT-DA)
The superior performance of deep models relies on the strong assumption that both training and testing data examples are drawn from identical data distribution. However, in real-world settings, the training data may not contain the prior knowledge of an infinite of testing scenarios, and thus models may encounter the issue of performance degradation when deployed at test-time, known as distribution shift. To improve model robustness against distribution shift, Domain Generalization (DG) aims to leverage one or multiple source domains to learn domain-invariant knowledge that could generalize well to any unseen target domain. Nevertheless, a lack of domain-specific knowledge of the target domain hinders the model from achieving the optimal. Instead, Test-time adaptation (TTA) allows the model to access unlabeled target data only at test-time, which enables the pre-trained model to adapt to the target domain before making predictions.

A well-designed mechanism for TTA-DA should carefully address two fundamental challenges. First, how to effectively encode domain-specific knowledge so that the semantic knowledge can remain untouchable during adaptation? Encoding knowledge in the model's parameter space, most conventional approaches select a subset of parameters to store domain knowledge. However, it is extremely hard to specify the subset and its size to achieve a balance between the limited adaptation capacity and overfitting with few-shot target data. Second, how to efficiently adapt the model with the domain knowledge given the limited unlabelled target data? Previous works craft unsupervised objectives, such as self-supervised auxiliary tasks or pseudo labels, to finetune the domain-related subset parameters, but heuristic unsupervised objectives may provide noisy supervision. In addition, finetuning a model after deployment at test-time requires extra abundant computation power and memory space and is thus unfriendly to resource-constrained devices. 

Alternatively, inspired by the success of prompting in NLP, Visual prompting can provide a novel framework for Test-Time Adaptation to address distribution shifts. In visual prompting, a large foundational model (FM)—pretrained on web-scale datasets (e.g.CLIP) and endowed with out-of-distribution generalization—can be steered to perform a downstream task by prepending prompt tokens to the image input instead of optimizing the entire network. Inspired by this, we encode domain-specific knowledge into a prompt and leave the semantic knowledge in the foundation model unspoiled. It assumes the highly generalized feature inherent in the foundation model can be manipulated to adapt to any domain by injecting corresponding domain-specific knowledge. This enables the modification of domain knowledge exclusively within the input space instead of the parameter space. The remaining challenge lies in how to effectively acquire a valid target domain prompt at test-time by combining the specific knowledge extracted from limited unlabeled target data with the shareable knowledge transferred from multi-source datasets. [ ]  first encodes the knowledge of multi-source domains into distinct domain prompts by learning from each source dataset independently, and then learns to aggregate these multiple source prompts into a target prompt by comparing the similarity with the target input feature. [ ] first heuristically partitions the domain prompt into domain-specific and domain-sharable components initialized by supervised learning on multi-source datasets, and then employs a manually designed regularization to preserve the domain-sharable component, thereby facilitating knowledge transfer in the adaptation.

However, these early attempts in visual prompting have multiple major drawbacks. First, both approaches finetune the FM on multi-source datasets, thereby violating the fundamental principle of prompting. This significantly hampers the FM’s intrinsic robustness in handling domain shifts. In addition, finetuning introduces prohibitive training costs and becomes extremely impractical as the size of FMs continues to grow. Second, both solely fullfill the objective of classification when learning the multi-source domain knowledge, potentially capturing shortcut patterns rather than the intrinsic data distribution in the source domain prompts. Last, the modeling process of multi-source domains and the scheme of test-time adaptation are separated into two distinct learning phases. This may not guarantee that the learned knowledge can be optimally transferable to a target domain.


We introduce XXX, a novel visual prompting approach that aims to extract domain-specific knowledge from limited unlabeled data to guide the foundation model to adapt to an unseen domain. Concretely, we propose a domain prompt generator in which a learnable knowledge bank is designed to encode transferable knowledge from multiple source domains. Given a target domain, the prompt generator takes as input a mini-batch of unlabeled data to condense the knowledge bank into a domain-specific prompt. To strengthen the domain knowledge condensation without semantic interference , we introduce a domain-aware contrastive loss to supervise the prompt generator. This also allows us to exploit large-scale unlabeled data only with domain IDs to further improve generalization. Moreover, the generated domain prompt is incorporated into the foundation model via a decoding module to guide the adaptation. To learn the knowledge bank, the process of knowledge transfer, and the process of guiding the foundation model simultaneously, we employ episodic learning to train the prompt generator and the decoder module at the meta-level. 

Our proposed method also provides additional practical advantages. As the domain prompt is the output embedding from the Prompt Generator, it is unnecessary to backpropagate the gradients through foundational model to optimize the prompt vectors in Prompt Tuning. This feature allows our Prompt Generator can be readily integrated with commercially available foundational models via APIs in black-box setting, significantly reducing memory overheads and privacy leak. Furthermore, generating a target domain prompt at test time is gradient-free, making it well-suited for on-device deployment scenarios.

We summarize our main contributions as follows: 1) We propose a novel test-time adaptation framework that is tailored to address distribution shifts. Our framework employs the concept of visual prompting and formulate the adaptation process as extracting domain-specific knowledge from unlabeled data into a prompt to guide the foundation model. 2) We design a visual prompt generation approach that aims to learn the process of domain knowledge extraction and decoding via meta-learning. Our method is also resource-efficient in training and deployment, as the large models can be treated as a black box without the need to access its internal information. 3) We conduct extensive experiments to show the superiority of the proposed method among the state-of-the-art and verify the effectiveness of each component. 




==> Old/Preliminaries_1.tex <==
\newpage
\section{Preliminaries1}
% In this section, we describe the problem setting and the motivations for our domain adaptive method. 

\noindent{\textbf{Problem setting.}} In this work, we follow the \hl{\textit{Test-time Domain Adaptation (TT-DA)}} as in~\citep{zhong2022meta}. Specifically, a dataset is comprised of \textit{N} source domains: $\mathcal{D}_s=\{\mathcal{D}_s^i\}_{i=1}^N$ and \textit{M} target domains: $\mathcal{D}_t=\{\mathcal{D}_t^j\}_{j=1}^M$. Each of the source domain contains labeled data: $\mathcal{D}_s^i = (x_s, y_s)^i$ while the target domains only have unlabeled data: $\mathcal{D}_t^j = (x_t)^j$. $(x, y)$ denote the input image and output label pair.  We assume distribution shift occurs between any pair of the source and target domains $\{\mathcal{D}_s^1, ..., \mathcal{D}_s^N, \mathcal{D}_t^1, ..., \mathcal{D}_t^M \}$, but all the domains share the same label space. TT-DA aims to perform training on the source domain data. When an unseen target domain $\mathcal{D}_t^j$ is encountered during testing (e.g., model deployed at a new scene), the trained model is expected to adapt to that particular domain using only \textbf{a small number of unlabeled data} (e.g., 16 images). The adapted model is then adopted for inference. TT-DA enforces mutual independence between source and target domains, accessing both types of domains is strictly prohibited. 

\noindent{\textbf{Motivations.}}  DG approaches~\citep{ghifary2015domain,li2018deep} normally expect an undifferentiated model to tackle myriad domain shifts in real-world which is manifestly less than ideal~\citep{zhong2022meta}. The reason behind the success of tackling domain shift in TT-DA methods is that a small amount of unlabeled data $\textbf{x}$ conveys the clue of target distribution $p(x)$~\citep{zhang2021adaptive}. Learning such underlying domain information plays a pivotal role in performance boost in estimating $p(y|x)$. However, two fundamental challenges should be carefully considered in TT-DA: 1) how to learn valid transferable knowledge from source domains?; 2) how to use these knowledge to guide the domain knowledge extraction from few-shot data \textbf{x}?


% 1) how to effectively extract the domain knowledge from $\textbf{x}$ which is sparsely sampled from $p(x)$?; 2) how to transfer the knowledge from the training source domains to assist the adaptation process? 

Meta-DMoE~\citep{zhong2022meta}, a representative gradient-based TT-DA approach, queries separate domain knowledge from source experts $\mathcal{M}$ using $\textbf{x}$. An aggregator then combines the knowledge and yield a supervision signal to distill the knowledge using loss $\mathcal{L}_{KD}$:
\begin{equation}
    \textbf{Y}' = f(\textbf{X}; \theta'), \quad \text{where} \quad \theta' = \theta - \alpha \nabla_\theta \mathcal{L}_{KD}(\textbf{x}, \mathcal{M}).
\end{equation}
$\textbf{X}$ and $\textbf{Y}'$ represent all the inputs and model predictions for that domain. $f(\cdot, \theta')$ denotes model parameterized by $\theta'$. $\textbf{x}$ is a small batch sampled from $\textbf{X}$ and $\alpha$ is the learning rate. 

% The supervision for adapting $\theta$ comes from an aggregator that combines knowledge from a group of pre-trained source domain experts. 

DoPrompt~\citep{zheng2022prompt}, a recent vision prompting-based approach ~\citep{jia2022visual} that adapts Vision Transformer (ViT)~\citep{dosovitskiy2020image} to every single image instance $x$ as: 

\begin{equation}
    y' = f([\,\texttt{[CLS]}, E(x), \textbf{P}'\,]), \quad \text{where} \quad \textbf{P}'= \sum_{n=1}^{N} w_n\textbf{p}_n, \quad \{w_1,...,w_N\} = \mathcal{A}(f(x)).
\end{equation}

$\texttt{[CLS]}$ is the class token, $E(x)$ is the image embedding. A set of prompts $\textbf{p}_*$ are trained on source domains. An input-dependent adapter $\mathcal{A}$ then generates weights $w_*$ to linearly combine  $\textbf{p}_*$ as $\textbf{P}'$.


% The pre-learned prompts on source domains $\textbf{p}_*$ are linearly combined by weights generated by an input-dependent adapter $\mathcal{A}$ to obtain adapted prompt $\textbf{P}'$. 

% In a high level sense, both DoPrompt and Meta-DMoE tackle the two above-mentioned challenges by two learning phases: 1) separately learn the domain-specific knowledge for each of the source domains with cross-entropy (CE) loss alone through vision prompts or expert models; 2) learning to combine and transfer the those source knowledge to unseen domains. The main limitation observed is that such independent two-stage training leads to non-purified domain information extraction on $\textbf{x}$. As the knowledge from each source domain is separately learnt via cross-entropy loss, each network/module may learn shortcut patterns to only fulfill classification instead of the intrinsic data distribution~\citep{li2023rethinking}. On the other hand, their optimization process does not impose intra-domain similarity and inter-domain discrepancy for the extracted information. 


In a high level sense, both DoPrompt and Meta-DMoE tackle the two above-mentioned challenges by two disjoint learning phases: 1) train separate vision prompts or expert models independently on source domains with cross-entropy (CE) loss.
2) learn to adapt towards unseen domains by combining those source knowledge. Several limitations are observed: in the initial learning phase, each network/prompt may learn shortcut patterns to only fulfill classification instead of the intrinsic data distribution~\citep{li2023rethinking}. Therefore, it is not guaranteed that the learned knowledge can be optimally transferable to unseen domains, leading to non-purified domain information extraction on $\textbf{x}$. Furthermore, both methods require weight updates at different learning stages. When migrating to more powerful foundation models (e.g., CLIP~\citep{radford2021learning}), the intrinsic robustness on handling domain shift can be significantly hampered~\citep{wortsman2022model}

% A range of drawbacks are observed: i) the two-phase learning, which is disjoint, does not ensure the source knowledge learned at first stage to be optimally transferable to unseen domains; ii) learning each of the source domain knowledge is independent, leading to redundant or conflicting information; iii) the optimization process does not impose intra-domain similarity and inter-domain discrepancy, leading to non-purified domain information extraction; iv) both methods require weight updates at different learning stages. When migrating to more powerful foundation models (e.g., CLIP~\citep{radford2021learning}), their intrinsic robustness on handling domain shift can be significantly hampered~\citep{wortsman2022model}

% iv) ineffective domain knowledge extraction


==> Old/intro_chi_1.tex <==
\section{Introduction}
% In this section, we describe Distribution Shifts, Domain Generalization, and our few-shot Test-time domain adaptation (FS-TT-DA)
The superior performance of deep models relies on identical distribution between training and testing data~\citep{choi2018stargan}. However, in the real world, expecting the training set to cover the universal distribution is practically unfeasible. Consequently, domain shift occurs at test time on unseen distributions, leading to performance deterioration~\citep{koh2021wilds}. To tackle distribution shift, Domain Generalization (DG), a line of research, aims to learn domain-invariant space from source domains that can generalize well across unseen target domains~\citep{pmlr-v28-muandet13, ghifary2015domain, balaji2018metareg}. Nevertheless, lacking specialized knowledge in the target domain can lead to flawed solutions~\citep{sun2020test}. In fact, a limited amount of unlabeled data from the target domain is readily accessible at test-time (e.g., image collection during camera calibration). Therefore, an additional learning phase is adopted to adapt the model towards \textit{each target domain} using those few-shot unlabeled data before inferences on remaining target data~\citep{zhong2022meta}.

Extracting domain knowledge from few-shot data remains a major obstacle. 
Hence, transferring knowledge from source domains to enhance such a process through correlated information is vital. To achieve this, three fundamental challenges should be carefully addressed: 1) how to effectively learn transferable knowledge from source domains to assist such a process? 2) how to acquire valid domain-specific knowledge for the target domain with the aid of learned source domain knowledge. 3) how to efficiently guide the trained model using the target domain-specific knowledge? \citep{zhong2022meta} encode the multi-source domain knowledge into a mixture of expert networks. A few unlabeled data is collected from a target domain to query the transferable knowledge that supervises the adaptation of a student network via fine-tuning. However, storing domain knowledge in the parameter space of expert networks introduces exorbitant computation and storage costs that grow linearly with the number of source domains~\citep{puigcerver2023sparse}. Moreover, updating the entire network at test-time is infeasible for resource-constrained devices~\citep{NEURIPS2020_81f7acab, NEURIPS2022_90c56c77}.

Alternatively, following the recent trend in Prompt Tuning~\citep{lester-etal-2021-power, li-liang-2021-prefix, liu2022p} in NLP, Visual Prompt Tuning (VPT)~\citep{bahng2022exploring, jia2022visual, Wang_2022_CVPR, wang2022dualprompt, han2023e2vpt} provides a parameter-efficient fine-tuning framework, by learning the prepended prompt tokens at the visual input space only instead of updating the entire network. VPT is adopted to efficiently handle distribution shifts, allowing the modification of domain knowledge exclusively within the input space instead of the parameter space~\citep{zheng2022prompt, gao2022visual, gan2023decorate}. \citep{zheng2022prompt} independently encode the knowledge of each source domain into distinct domain prompts. A target prompt is then produced by linearly combining the pre-learned source domain prompts. \citep{gan2023decorate} learn source domain prompts via supervised learning and heuristically partition them into domain-specific and domain-shareable components. To facilitate knowledge transfer during adaptation, a manually crafted regularization term is employed to preserve the domain-shareable part while allowing the domain-specific component updates.


However, several major drawbacks are observed. First, they model the source domain knowledge by minimizing the cross-entropy loss solely. The domain prompt may inadvertently learn semantic patterns as a shortcut to fulfill the classification task instead of learning intrinsic source distribution~\citep{li2023rethinking}. Second, separating the process of modeling source knowledge and the process of learning to adapt into independent training phases may compromise optimal knowledge transfer to the target domain. Last, they opt to finetune the backbone network on source domain data for the performance boost. Such finetuning incurs prohibitive training costs~\citep{pmlr-v202-dehghani23a}.


In this work, we propose a novel approach to incorporate the visual prompt and the large Foundation Models (FMs) ~\citep{bommasani2021opportunities} (e.g., CLIP \citep{radford2021learning}) to address distribution shifts. The FMs, trained on web-scale data, exhibit robust generalized features~\citep{Wortsman_2022_CVPR}. We contend that with proper guidance, such generalized visual features can boost the model's performance on a specific data distribution. Thus, we propose to build adaptation on top of their features while keeping their inherent robustness unspoiled. Our key idea is to generate a domain-specific visual prompt from few-shot unlabeled data and manipulate the FM features to provide guidance to the FMs. Specifically, we propose a domain prompt generator in which a learnable knowledge bank is designed to encode transferable knowledge from source domains. Given a target domain, our prompt generator treats a mini-batch of unlabeled data as a condition to condense the knowledge bank into a domain-specific prompt. This generated domain prompt is then incorporated into the FM features via a guidance module for subsequent inference. To purify the domain-specific knowledge and reduce semantic interference, we introduce a domain-aware contrastive loss to enhance the prompt generator. This also allows us to further elevate the generator by exploiting large-scale unlabeled data with only domain IDs~\citep{sagawa2022extending}. Moreover, to learn the transferable knowledge and the mechanism of adaptation simultaneously, we employ episodic learning to align the learning objectives of the prompt generator and the guidance module at the meta-level~\citep{hospedales2021meta}.  
 
Our proposed method also provides additional practical advantages. All of our modules work on the output feature of the FMs without access to the FM's weights. It allows our method to be readily integrated with commercially available FMs via APIs in a black-box setting~\citep{ouali2023black}, significantly reducing memory overheads and privacy leaks \citep{xu2020information}. 
Furthermore, generating a target domain prompt at test-time is gradient-free, making it well-suited for on-device deployment scenarios.

We dub our method as \textbf{V}isual domain \textbf{P}rompt \textbf{G}enerator (VPG), and summarize our main contributions as follows: 1) We propose a novel approach that employs the visual prompt and the foundation model to tackle distribution shifts. Our approach formulates the adaptation process as generating a visual prompt that encodes domain-specific knowledge to guide the foundational model. 2) we propose domain-aware contrastive loss and episodic learning to enhance the domain knowledge generation.
% 2) Our method offers multiple practical benefits, including computational efficiency, low memory consumption during both training and deployment, and privacy guarantee 
3) We conduct extensive experiments to show the superiority of the proposed method among the state-of-the-art and verify the effectiveness of each component. 
 



